FlooNoC: A 645 Gbps/link 0.15 pJ/B/hop Open-Source NoC with Wide Physical Links and End-to-End AXI4 Parallel Multi-Stream Support

The new generation of domain-specific AI accelerators is characterized by rapidly increasing demands for bulk data transfers, as opposed to small, latency-critical cache line transfers typical of traditional cache-coherent systems. In this paper, we address this critical need by introducing the FlooNoC Network-on-Chip (NoC), featuring very wide, fully Advanced eXtensible Interface (AXI4) compliant links designed to meet the massive bandwidth needs at high energy efficiency. At the transport level, non-blocking transactions are supported for latency tolerance. Additionally, a novel end-to-end ordering approach for AXI4, enabled by a multi-stream capable Direct Memory Access (DMA) engine simplifies network interfaces and eliminates inter-stream dependencies. Furthermore, dedicated physical links are instantiated for short, latency-critical messages. A complete end-to-end reference implementation in 12nm FinFET technology demonstrates the physical feasibility and power performance area (PPA) benefits of our approach. Utilizing wide links on high levels of metal, we achieve a bandwidth of 645 Gbps per link and a total aggregate bandwidth of 103 Tbps for an 8x4 mesh of processors cluster tiles, with a total of 288 RISC-V cores. The NoC imposes a minimal area overhead of only 3.5% per compute tile and achieves a leading-edge energy efficiency of 0.15 pJ/B/hop at 0.8 V. Compared to state-of-the-art NoCs, our system offers three times the energy efficiency and more than double the link bandwidth. Furthermore, compared to a traditional AXI4-based multi-layer interconnect, our NoC achieves a 30% reduction in area, corresponding to a 47% increase in GFLOPSDP within the same floorplan.

==> figures/tech_scaling.tex <==
\begin{figure}[h]
\centering
    \begin{tikzpicture}[scale=1.1]
    \begin{axis}[
        % title={Technology Scaling of On-Chip Wire Resources},
        % xlabel={Technology Generation},
        ylabel={Min. Metal Pitch [\SI{}{\nano\meter}]},
        axis y line*=left,
        xmin=0.5, xmax=10.5,
        ymin=0, ymax=220,
        xticklabels={\SI{65}{\nano\meter},\SI{45}{\nano\meter},\SI{32}{\nano\meter  },\SI{22}{\nano\meter},\SI{14}{\nano\meter},\SI{10}{\nano\meter}, \SI{7}{\nano\meter}, \SI{5}{\nano\meter}, \SI{3}{\nano\meter}, \SI{2}{\nano\meter}},xtick={1,...,11},
        ytick={50,100,150,200,250,300},
        xticklabel style = {xshift=0.5ex, rotate=60, anchor=east},
        yticklabel style = {font=\footnotesize},
    ]
    
    % Dummy data for minimal metal pitch
    \addplot[color=PULPBlue,mark=square]
        coordinates {
        (1,210)(2,160)(3,115)(4,72)(5,56)(6,36)(7,36)(8,30)(9,24)(10,20)
        }; \label{metal_pitch}
    
    \end{axis}
    
    \begin{axis}[
        axis y line*=right,
        axis x line=none,
        ylabel={Number of Interconnect Layers},
        xmin=0.5, xmax=10.5,
        ymin=7, ymax=18,
        ytick={4,6,8,10,12,14,16,18},
        yticklabel style = {font=\footnotesize},
        legend style={at={(axis cs:6, 12)},anchor=west}
    ]
    
    \addlegendimage{/pgfplots/refstyle=metal_pitch}\addlegendentry{pitch}
    
    % Dummy data for number of interconnect layers
    \addplot[color=PULPOrange, mark=triangle]
        coordinates {
        (1,8)(2,9)(3,9)(4,9)(5,13)(6,14)(7, 15)(8, 15)(9, 17)(10, 17)
        };
    
    \addlegendentry{\#layers}
    % \addlegendentry{\ref{metal_pitch} bubu}
    
    \end{axis}
    \end{tikzpicture}
\caption{Technology scaling of on-chip wire resources based on IDRS reports \cite{IRDS2016, IRDS2017, IRDS2018, IRDS2021, IRDS2022} for 2-\SI{14}{\nano\meter}\cite{interco_scaling16} and for 22-\SI{65}{\nano\meter}}
\label{fig:tech_scaling}
\end{figure}
